RefChecker: Reference-based Fine-grained Hallucination Checker and Benchmark for Large Language Models

Large Language Models (LLMs) have shown impressive capabilities but also a concerning tendency to hallucinate. This paper presents RefChecker, a framework that introduces claim-triplets to represent claims in LLM responses, aiming to detect fine-grained hallucinations. In RefChecker, an extractor generates claim-triplets from a response, which are then evaluated by a checker against a reference. We delineate three task settings: Zero, Noisy and Accurate Context, to reflect various real-world use cases. We curated a benchmark spanning various NLP tasks and annotated 11k claim-triplets from 2.1k responses by seven LLMs. RefChecker supports both proprietary and open-source models as the extractor and checker. Experiments demonstrate that claim-triplets enable superior hallucination detection, compared to other granularities such as response, sentence and sub-sentence level claims. RefChecker outperforms prior methods by 6.8 to 26.1 points on our benchmark and the checking results of RefChecker are strongly aligned with human judgments. This work is open sourced at https://github.com/amazon-science/RefChecker

==> sections/01intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

Large Language Models (LLMs) have sparked a revolution in Natural Language Processing (NLP), covering diverse tasks with a unified architecture\cite{LLMSurvey}. However, LLMs exhibit a tendency to generate hallucinated contents that can be challenging to discern, possibly leading users astray\cite{huang2023survey}. 
Hallucination detecting is therefore an important task\cite{manakul-etal-2023-selfcheckgpt, min-etal-2023-factscore, chern2023factool}. 
%Consequently, it is important to identify these hallucinations within LLM-generated responses, pivotal for wider adoption of LLMs. To address this, our study centers on the construction of a standardized assessment framework aim to identify such hallucinations present in the outputs of LLMs.

% Despite the importance of the problem, there has not been a more rigorous definition \pfliu{``definition of what?''}and, as a consequence, there exist a myriad of confusions. For instance, LLMs are general purposes and are capable of performing a variety of tasks, with different contexts available at the time of inference, which influences the degree and source of hallucination. Second, some hallucinations are more “harmful” than others, and we need a more principled way of categorizing them. Finally, our everyday experience reveals that partial hallucination is common, meaning only some of the information are faulty. This poses a significant challenge as how to design the unit (or granularity) of checking. Without a clear definition of the granularity and the types of hallucination, it will be meaningless to advance the study.\pfliu{what's our solution?}
%\zz{LLM can hallucinate by generating non-factual pieces of information, or corrupt information even when it is provided in the context.}
%To address this problem, several challenges must be confronted. Firstly, LLMs exhibit a broad range of capabilities, making them versatile for various tasks. However, this versatility ijtroduces the risk of producing diverse types of hallucinations across different tasks.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/claim_dist_llama2.pdf}
    \caption{Llama2's responses on our benchmark, broken into three groups based on the number of claim-triplets they contain, and their ratios across categories.}
    \label{fig:claim_dist}
    \vspace{-15pt}
\end{figure}
The very versatility of LLM leads to the complexity of hallucination detection.
%LLM responses can contain non-factual pieces information, or corrupt information even when it is provided in the context. 
For example, we would expect the least amount of hallucination in translation and a lot more in closed book fact-seeking tasks, and the nature of the hallucination will also differ. In other words, 
both the types and the degree of hallucination correlates strongly with the availability of context in a given task.  

Our first contribution is to curate a comprehensive dataset that we can benchmark hallucination depending on whether references are given and their quality (see Table~\ref{tab:compare_related_work}). Indeed, as expected, we found hallucination is the most pronounced when LLMs are asked to generate responses solely from its memory, followed by responding to noisy references in RAG (retrieval augmented generation) setting\cite{gao2024retrievalaugmented}, and finally when references are more or less noisy free (cf. Appendix~\ref{appendix:observation_from_human_eval}).

\zz{next contribution, KG -- 1/ total annotations, impress with the quantity of work, 2/ necessity by fig-1, is there a better way? 3/ adv, 15pt(?) better than response and xpt than sentences, subsentences}

\zz{next contribution, framework intro, emphasize on open LLMs}

%Conversely, in fact-seeking tasks we are asking the model to generate from (potentially stale) internal memory and expect to see more hallucinations. 
% Therefore, \rc begins by partitioning the hallucination detection landscape by the availability and quality of contexts, and curate representative benchmarks, as follows (also see Table~\ref{tab:benchmark_data}):
%\zz{now talk about zero, accurate and noisy context, leaving factuality vs faithfulness in the related work}. 
% \begin{itemize}[noitemsep,topsep=1pt,leftmargin=1pt,itemindent=1pc]
%     \item Zero Context (ZC): Tasks in this setting require the LLM to respond solely based on its internal knowledge. Therefore, in principle, references should be in the training corpus. In practise, we need a proxy dataset to represent such stable knowledge. 
%     %We utilize fact-seeking questions sourced from Natural Questions (NQ) as the benchmark. Ideally, the reference would come from the LLM's training data, since this reflects the knowledge it has learned. However, due to limitations with proprietary models, this is often not feasible. As a proxy, we use the human-annotated long answers in NQ as the reference.

%     \item Noisy Context (NC): In this setup, the LLM receives additional context retrieved from some external knowledge source, which may contain noisy or irrelevant information. NC is also known as Retrieval-Augmented Generation (RAG), a crucial use case frequently encountered in real-world applications. %We sample examples from MS MARCO, one of the standard datasets for RAG, as the benchmark for NC, and take the input context as the reference.

%     \item Accurate Context (AC): This setting is similar to NC but the reference is typically noise-free. Examples include text summarization, closed-QA and information extraction tasks.
%     %In this scenario, the context is directly given by the user as in tasks like summarization, ensuring the context is clean and accurate compared that in NC. We take a subset of Dolly-15k instruction tuning dataset as the benchmark for AC, covering text summarization, closed-QA and information extraction tasks, to reflect diverse use cases. Similar to NC, the input context serves as the reference for detecting hallucinations.

% \end{itemize}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/refchecker_pipeline.png}
    \caption{The \rc pipeline comprises two main components: an extractor denoted as $E$ and a checker denoted as $C$. Given a text to be checked, typically a response generated by a LLM, the extractor takes it as input and generates a set of knowledge triplets, referred to as claim-triplets. Subsequently, the checker assesses each claim-triplet by comparing it against a reference, assigning a hallucination label based on the evaluation.}
    \label{fig:refchecker_pipeline}
    \vspace{-15pt}
\end{figure*}

% By grouping different tasks according to the availability and quality of context, it becomes easier to examine and compare hallucinations across tasks. As we will report in Appendix~\ref{appendix:observation_from_human_eval}, hallucinations indeed increase from AC to NC and finally to ZC. The partition also meaningfully unifies and extends existing definitions in \citet{huang2023survey}: factuality hallucination maps to AC, whereas faithfulness is broken down to NC and AC, each has a group of important tasks. Our future work includes expanding more tasks in each of the partition.

% the text below can be moved into related work
%\textbf{Factuality Hallucinations} manifest when an LLM responds to a factual question based on its internal knowledge, resulting in responses that contradict established real-world facts. For instance, when queried about the capital of France, the LLM may erroneously assert "London". Factuality hallucinations are also aligned with the main focus of Fact-Checking\cite{guo-etal-2022-survey}. On the other hand, \textbf{Faithfulness Hallucinations} arise when an LLM, provided with a context, generates an output that deviates from the fidelity expected within that context. For example, when tasked with summarizing a news article, the LLM should not distort the content of the news to maintain faithfulness to the original context. However, to the best of our knowledge, current works predominantly focus on the detecting factuality hallucinations\cite{manakul-etal-2023-selfcheckgpt, min-etal-2023-factscore, chern2023factool}, while a holistic approach addressing both factuality and faithfulness hallucinations remains absent. 

% simplify the text below.
Detecting hallucination is essentially a job of comparing a response against a reference (or a set of them in RAG/NC setting). If the query is about a simple fact and the response is straightforward, response level checking~\cite{lin-etal-2022-truthfulqa, li-etal-2023-halueval} suffices. In the benchmarks we curated, both references and responses can be complex and long. 
%For instance, responses of GPT-4 contain 28, 44, and 50 tokens on average in the zero-, noisy- and accurate-context setting. 
Thus, extending various approaches that perform detection at finer granularity~\cite{manakul-etal-2023-selfcheckgpt, min-etal-2023-factscore, chern2023factool}, \rc extracts knowledge triplets as checking units. These triplets are called \textit{claim-triplets}. 
%The RefChecker pipeline starts by extracting such triplets, called \textit{claim triplets}, using an LLM (fig~\ref{}). 
A typical response contain multiple triplets with various factuality. Figure~\ref{fig:claim_dist} groups Llama2's responses on our benchmark into different bins according to numbers of claim-triplets they contain, and depicts the categorical distribution of the triplets (introduced next). A response-level checker will miss all these details.
%plots the label ratios of claim-triplets in Llama2's response relative to their numbers, breaking down into different . This  analysis reveals that responses encompass numerous claims, with varying degrees of hallucination.



%Secondly, everyday experiences demonstrate that partial hallucination is a prevalent occurrence, wherein only specific pieces of information are erroneous. This poses a substantial challenge in determining the appropriate unit or granularity for conducting checks. Response-level checking\cite{lin-etal-2022-truthfulqa, li-etal-2023-halueval} follows a straightforward pipeline, but its results are inherently coarse-grained. In an effort to identify finer-grained hallucinations, \citet{manakul-etal-2023-selfcheckgpt} introduced sentence-level detection, involving the examination of individual sentences within a response. However, this approach may overlook hallucinations that span across sentences. Addressing this challenge, \citet{min-etal-2023-factscore} and \citet{chern2023factool} propose a strategy wherein claims extracted from the response serve as the checking units. Nevertheless, the granularity of these extracted claims remains unclear, as they are generated by LLMs with in-context demonstrations.

This formulation affords us to apply the familiar entailment framework to check claims within an LLM response. In this framework, an \textit{entailed} claim is corroborated directly by the reference, a \textit{contradictory} claim is refuted otherwise, and a \textit{neutral} claim is one that cannot be confirmed or denied by the reference. Checking at this granularity makes it trivial to map to response-level checking, whereas the reverse is difficult. For instance in the most strict setting a response is contradictory as long as any one claim triplet is contradictory. 
% reuse the following if you can
%Thirdly, it is crucial to recognize that not all hallucinations carry the same degree of potential harm, underscoring the need for a more nuanced categorization system. Existing approaches to factuality hallucination detection often employ a binary classification, distinguishing between factual and non-factual claims in comparison to the references. However, in real-world applications, references may not consistently offer adequate evidence to validate all claims. Therefore, a more sophisticated categorization framework is essential to capture the varied nature of hallucinations.

% Lastly, the establishment of a standard benchmark becomes imperative. This benchmark would not only serve for assessing how LLMs engage in hallucination but also evaluating the performance of hallucination detection approaches in addressing this problem. Previous benchmarks are either for factuality hallucination only, or have a narrow domain and task coverage. 

%zz you can use them to earlier
%Lastly, it is crucial to establish a standardized benchmark. This benchmark serves the purpose of evaluating the extent to which LLMs exhibit hallucination and assessing the efficacy of hallucination detection approaches. Existing benchmarks primarily focus on factuality hallucination or have limited coverage across specific domains and tasks. A comprehensive and widely applicable benchmark is essential for a more thorough evaluation of LLMs and the methods employed for hallucination detection.

The \rc pipeline is composed by pairing up an extractor and a checker, as shown in Fig~\ref{fig:refchecker_pipeline}. This pipeline is built progressively as we gain experience. After we curated the dataset and responses of 7 initial LLMs, we performed manual annotation of the claim-triplets extracted by Claude 2, for a total of 2100 responses and 11k triplets (Section~\ref{sec:taxonomy}). These annotations are then used to study, develop and calibrate a suite of proprietary and open-source LLM based extractors (Section~\ref{sec:pipeline_extractor}) and checkers (Section~\ref{sec:pipeline_checker}) to arrive at a fully automated and model-based hallucination detection pipeline. We made careful study to select and recommend configurations that give results consistent with human annotation, and show 19 to 26 points of improvement over the best alternative (Section~\ref{sec:compare_other_approach}). %The project is open sourced and available at \footnote{link}

%with recommended configurations that gives results consistent with human annotation. Lastly, leveraging the Mistral/Mixtral suite, we make RefChecker based entirely on open LLMs, with performance that rivals the best of proprietary LLM-based extractor/checker combinations.

%To summarize, RefChecker makes the following contribution:

%In this paper, we present RefChecker, a hallucination detection framework designed to address these challenges. We delineate three distinct task settings: Zero Context, Noisy Context, and Accurate Context, aiming to differentiate the contextual conditions under which the user queries are posed. Encompassing Zero Context for factuality, and Noisy and Accurate Context for faithfulness hallucinations, these three settings collectively span a diverse array of real-world use cases. 

%The RefChecker pipeline, depicted in Figure~\ref{fig:refchecker_pipeline}, employs a novel approach for representing claims through knowledge triplets, referred to as \emph{Claim-Triplets}. These triplets are extracted by an \emph{Extractor}, drawing inspiration from the field of knowledge graph studies, where triplets are utilized to encapsulate factual knowledge units. Subsequently, each claim-triplet undergoes evaluation by the \emph{Checker} to compare it with a reference. The evaluation process includes classification with a hallucination label, which not only considers whether the claim is factual or not but also evaluates its verifiability based on the given reference. 

% We assembled a benchmark dataset covering the three setting mentioned above and spans a broad range of NLP tasks. With this benchmark, we evaluated seven LLMs and conducted human evaluations on the claim-triplets. We developed an automatic checking pipeline based on both proprietary and open-sourced models. As a result, we totally annotated 11k claim-triplets within 2.1k collected responses. Our experiments show that RefChecker achieves better performance on our benchmark compared with previous methods, and using claim-triplets reveal superior performance of hallucination detection compared with other granularities. 


%We curated a comprehensive benchmark dataset that encompasses three distinct settings and spans a diverse array of NLP tasks. On this benchmark, we assessed the performance of seven LLMs and conducted human evaluations on 11k claim-triplets across 2,100 gathered responses.

%We developed an automatic pipeline leveraging both proprietary and open-sourced models. Our experiments demonstrate that RefChecker outperforms previous methods on our benchmark. Furthermore, employing claim-triplets as the claims reveals superior performance in hallucination detection compared to other levels of granularity.

==> sections/06experiments_backup.tex <==
\section{Experiments}

To show how well RefChecker performs on hallucination detection tasks, we conduct experiments to evaluate the extractors and checkers, respectively, and evaluate the whole pipeline with ranking correlations against human evaluation.

\subsection{Evaluation on Extractors}
\label{sec:exp:extractor-eval}
\input{tables/extractor_evaluation_comparison} 
For accurate hallucination detection, we need to first extract high-quality claims that express facts in the original response as faithfully and completely as possible. However, the evaluation of claim extraction is non-trivial due to the diverse expressions of the same fact. To alleviate the burden of post-hoc human evaluation for each extractor, we adopt an automatic evaluation pipeline using GPT-4 Turbo (\texttt{gpt-4-1106-preview}).

We prompt GPT-4 Turbo to attach a \texttt{True/False} flag to each extracted claim, which indicates whether the claim faithfully express original semantics in the response. We also prompt it to complete missing claims. This way, 
%With results above, 
we can automatically calculate the \textbf{precision}, \textbf{recall}, and \textbf{F1} score of extracted claims.
% Table~\ref{tab:extractor-evaluation-comparison} shows the results on randomly sampled 180 responses. 
%We use them o measure the extraction quality. We  from our benchmark as the test set for evaluation.
For a sanity check, we also repeated the process above with human evaluation on 30 random samples. When evaluating recall, we ask human annotators to first check whether each completed triplet in GPT-4 Turbo's output is correct or not, then completing more if there are still missing ones. It helps the computation of agreement between model and human evaluators. As shown in Table~\ref{tab:extractor-evaluation-comparison}, the overall evaluation by human and the automatic pipeline align well on the three extractors. They achieved 93.7\% agreement on precision and 91.9\% agreement on recall.

\input{tables/extractor_auto_results}


Given the reliability of the automatic evaluation pipeline, we demonstrated the performance of 4 extractors as in Table~\ref{tab:extractor-auto-results}. Our open-source Mistral extractor achieves near Claude 2 extraction quality with significantly faster inference speed and doesn't require API tokens.
\input{tables/checker_evaluation_main_results} 

\subsection{Evaluation on Checkers}
\label{sec:exp:checker-eval}

%\zz{after looking at the table, this is the conclusion I can draw }
%We evaluate the performance of various checkers against our annotations (Table~\ref{tab:checker_main}). Among the baseline checkers, AlignScore is a strong competitor to GPT-4. Finetuned Mistral checkers can often gives the best performance, though there does not yet exist a single winner across the board.

%As mentioned previously, our benchmark contains 2100 manual labeled responses with 11k fine-grained claim triplet labels. In this section, we use triplet-level labels to evaluate the performance of Mistral-based checkers against baseline checkers. 
%The evaluation metric is accuracy and macro-f1 score over 3-way classification.

As described in Section~\ref{sec:pipeline_checker}, the baseline checkers we include in the evaluation are RoBERTa-NLI, AlignScore, GPT-4 and Claude 2. The Mistral-based checkers we include are zero-shot prompted, one-shot prompted, LoRA fine-tuned and RepC-LE variants. The training and development data of these variants are 4k samples from the ANLI dataset \cite{nie2020adversarial}. We evaluate their performance using the 11k manually annotated claim triplets. The evaluation metric is accuracy and macro-f1 score over 3-way classification.



Table~\ref{tab:checker_main} shows the evaluation results. Among the baseline checkers, AlignScore is a strong competitor to GPT-4, and Claude 2 lags behind interestingly. We case study the results, and found Claude 2's neutral F1 score is very low (less than 20\%). Maybe understanding the concept of neutral is not trivial for Claude 2 without demonstration. 


Besides, the Mistral-based checkers can often gives the best performance, though there does not yet exist a single winner across the board. The weakness of Mistral-based checkers lies in the NC setting. A possible reason is that the training data of Mistral-based checkers are short paragraphs (less than 100 tokens) while in NC the reference can be very long (thousands of tokens). Therefore, we have to split the reference to fit the training data distribution and aggregate the predictions later. We will leave this part for future exploration.

\subsection{Evaluation on \rc Pipeline}
\label{sec:pipeline-perf}

%To validate the reliability of \rc in quantifying hallucinations across different LLMs, we use it to check responses on our benchmark grouped by the 7 responding LLMs. 
To validate the robustness and reliability of \rc, we checked 7 LLMs responses on our benchmark and compared rankings (ratios macro-averaged on responses of each LLM) by \rc and by humans with the Spearman's rank correlation coefficient. The entire configuration space consists of different combinations of extractor and checker, and also the 3 task settings as well as their averages. The results are reported in in Figure~\ref{fig:correlation}.

%We can find best configurations of \rc 
%have some recommendations on the use of \rc 
%based on the statistics in Figure~\ref{fig:correlation}. 
We find that Claude 2 extractor and GPT-4 checker combination is the most competitive option with \textit{very strong} correlations in all settings, benefiting from more powerful LLMs. Replacing the extractor with our Mistral alternative has slight drop of performance, maintaining \textit{very strong} correlations in most settings. The most economical and efficient option in our framework, the Mistral extractor (7B) and NLI/AlignScore checker (356M), still achieve consistently \textit{strong} correlations in all settings. The Mistral-RepC checker is robust against different extractors, owing to its stronger reasoning capability than small NLI-based checker. This result serves as an index to select a configuration per user's preference (e.g. budget, ease of deployment, a particular setting and types of hallucination).
%like the GPT-4 checker, demonstrating strong correlations when combined with any extractor.


\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/correlation.png}
    \caption{Spearman's rank correlation coefficients between \rc and human evaluation. Results are grouped regarding extractors and checkers used. Results for each extractor (column) and checker (row) are arranged into a sub-matrix in the figure, with values for 4 context settings (one additional for average) and 3 ranking metrics.}
    \label{fig:correlation}
    \vspace{-15pt}
\end{figure}

==> sections/07analysis_backup.tex <==
\section{Analysis}

\subsection{Comparing with Other Granularities}
\label{sec:compare_other_granularities}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/checker_granularity.pdf}
    \caption{Performance statistics of 7 checkers under different claim granularities on 2.1k manual annotated responses. The detailed checker performance can be found in Table~\ref{tab:granularity} of Appendix~\ref{appendix:refchecker_checker}.}
    \label{fig:checker_gran}
    \vspace{-15pt}
\end{figure}

Previous work used different claim granularity for hallucination detection, including response, sentence and sub-sentence levels (cf. Sec.~\ref{sec:related_work} and~\ref{sec:claim_triplet}). 
%Obviously, finer-granularity checking detects hallucination at a much higher resolution. Interestingly, we discover that even we aggregate triplet-level results into response-level, \zz{let's discuss, i don't understand how this is done}
We compare them with claim-triplets to verify the effectiveness of checking on facts with the triplet format.

To make the results with different granularities comparable to each other, we first breakdown the 2.1k annotated responses into different granularities,
then collect corresponding checker predictions respectively, and finally aggregate finer-level results all into the response-level. We utilize a strict aggregation rule with zero-tolerance on hallucinations, which means we apply max-pooling (Entailment $<$ Neutral $<$ Contradiction) over claim predictions within a response. We compare the results of 7 checkers, including 4 baseline checkers and 3 RepC-LS checkers, with macro-f1 on the three categories. As shown in Figure~\ref{fig:checker_gran}, triplet-level claims exhibit obvious superiority over other granularities.

% To compare checkers' performance at triplet-level against other granularities, we first break down the 2100 annotated responses into sentence and sub-sentence level claims as illustrated in~\ref{}. Then we feed them together with response and triplet level claims into checkers to obtain predictions in four granularities for each response. Afterwards, we align the granularities by merging checkers' predictions and manual triplet-level labels to response-level. Finally, with the response-level predictions and labels, we can compare the performance of each model under different claim granularities. The merge rule \lin{TODO}

% Figure~\ref{fig:checker_gran} shows the performance comparison results.
% We can see that using triplet-level granularity achieves the best average performance.

\subsection{Comparing with Other Approaches}
\label{sec:compare_other_approach}

\begin{table*}[!ht]\small
    \centering
    \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{2}{c}{Zero Context} & \multicolumn{2}{c}{Noisy Context} & \multicolumn{2}{c}{Accurate Context} \\
 & Pearson & Spearman & Pearson & Spearman & Pearson & Spearman \\ \hline
SelfCheckGPT & 35.40 & 43.15 & 36.31 & 32.15  & 40.23 & 32.55 \\
FActScore & 42.58 & 45.60 & 33.36 & 29.91 & 27.80 & 27.05 \\
FacTool & 59.78 & 62.57 & 46.35 & 38.69 & 31.41 & 32.82 \\ \hline
% \rc & \textbf{\textcolor{red}{83.95}} & \textbf{\textcolor{red}{82.35}} & \textbf{\textcolor{blue}{67.29}} & \textbf{\textcolor{blue}{59.94}} & \textbf{\textcolor{orange}{60.99}} & \textbf{\textcolor{orange}{58.96}} \\
\rc \\
\textit{GPT-4 + GPT-4} & \textbf{83.95} & \textbf{82.35} & \textbf{64.56} & \textbf{57.30} & \textbf{58.61} & \textbf{55.50} \\
\textit{Mistral-SFT + AlignScore} & \textbf{\textcolor{purple}{75.81}} & \textbf{\textcolor{purple}{74.16}} & \textbf{\textcolor{purple}{53.88}} & \textbf{\textcolor{purple}{45.09}} & \textbf{\textcolor{purple}{46.34}} & \textbf{\textcolor{purple}{43.22}} \\
\bottomrule
    \end{tabular}
    \caption{Automated checking results of \rc and previous approaches. The results of \rc are from the best performing combinations (extractor + checker) of proprietary LLMs and pure open-source models (purple colored numbers).}
    \label{tab:comapre_related_work_correlation_our_benchmark}
    \vspace{-15pt}
\end{table*}

As in Sec.\ref{sec:pipeline-perf}, we compare \rc against other alternatives by rank correlations produced by detection results. We pick three popular approaches, SelfCheckGPT~\cite{manakul-etal-2023-selfcheckgpt}, FActScore~\cite{min-etal-2023-factscore} and FacTool~\cite{chern2023factool}. These approaches use different metrics and we convert them as ``hallucination rates'', as follows:
\begin{itemize}[noitemsep, leftmargin=1pt, itemindent=1pc, topsep=1pt]
    \item SelfCheckGPT: the average score of the sentences within a response. The score is 0 for an \texttt{accurate} sentence, 0.5 for \texttt{minor\_inaccurate}, and 1 for \texttt{major\_inaccurate}.
    \item FactScore/FacTool: the proportion of claims not supported (FactScore) or non-factual (FacTool) by the reference.
    %\item FacTool: the proportion of non-factual claims.
    \item \rc: the proportion of Neutral and Contradiction claims. %we report two options, hallucination is either contradiction, or additionally include neutral.
\end{itemize}

The results show that \rc significantly outperforms previous methods across all three context settings with both proprietary and open-source models. We additionally apply \rc to SelfCheckGPT's dataset, and observe that in 11 out of the 15 combinations (73\%) of \rc outperform SelfCheckGPT. However, the numbers still indicate a great improve space, especially in NC and AC settings.

%To assess the efficacy of \rc in comparison to prior methodologies on our benchmark dataset, we conducted automated evaluations on the responses previously assessed by human judges\footnote{InstructGPT's responses were excluded from this comparison due to the unavailability of its API, which impedes the evaluation of SelfCheckGPT.}. We then analyzed the Pearson and Spearman's rank correlations between the "hallucination rates" of these responses and human annotations. The hallucination rate is determined differently for each method: for SelfCheckGPT, it represents the average scores of sentences within a response as per its definition; for FActScore and FacTool, it signifies the proportion of non-factual claims; for \rc, it denotes the rates of Neutral and Contradiction claims. Table~\ref{tab:comapre_related_work_correlation_our_benchmark} illustrates that \rc significantly outperforms previous methods across all three evaluation scenarios. Further detailed results are available in Appendix~\ref{appendix:compare_other_methods}, where \rc also demonstrates superior performance compared to SelfCheckGPT on the SelfCheckGPT dataset.









\subsection{Limitations and Future Work}

% \dyru{to be moved to a dedicated section which will not count toward the page limit}
% \xiangkun{Discussed with Dongyu, maybe we can summarize the results of case study here and points to the bias analysis in appendix conducted by Yun Luo}

There remain several limitations of \rc that require addressing:
\textbf{a)} The triplet format of claims, while effectively breaking down LLM responses into finer granularity, can be overly restrictive and may not have the flexibility to cover important semantics (consider \texttt{(Trump, president of, US)}, which is factual in 2018, but non-factual in 2022). 
%cannot cover all complex semantics in text. Enhancing expressiveness by incorporating quantifiers or attributes may result in a more robust format of claims.
\textbf{b)} While extraction is relatively simple with the outstanding comprehension capability of LLMs, there exists a large improvement space for more powerful checkers.
\textbf{c)} \rc has a rudimentary support for source attribution (see Appendix~\ref{appendix:refchecker:source_attribution}). Better source attribution is critical to lend explainable and provide training signal to mitigate hallucination.
%crucial for a hallucination detection system. Users seek information on where the hallucination occurs and supporting evidence in the reference, rather than just receiving verdicts.
\textbf{d)} We found that model-based checkers may exhibit bias towards internal knowledge, declaring a neutral claim to be entailment. This requires we inject some forms of ``source control'' in LLMs. 
%Investigating methods to constrain checkers to predict solely based on the provided reference or control them for a desired balance between internal and external knowledge is an interesting topic.
\textbf{e)} In actual deployment cases, we found users ask for stronger customizability (e.g. they would like to use \rc with their own database for reference retrieval) and speed improvement.
Appendix~\ref{appendix:limitations} discusses some of them in more detail.
%A more detailed discussion, including cases or quantitative results, is provided in Appendix~\ref{appendix:limitations}.

==> sections/backup05benchmark.tex <==
\section{Benchmark}

\begin{table*}[]\small
    \centering
    \begin{tabular}{lccc}
    \toprule
Setting & Data Source & Task & Reference  \\
\hline
Zero Context & \makecell{NaturalQuestions\\(development set)}  & Closed Book QA & Annotated Long Answer  \\
\hline
Noisy Context & \makecell{MS MARCO\\(validation set)} & \makecell{Retrieval-Augmented Generation\\(RAG)} & Retrieved Passages \\
\hline
Accurate Context & databricks-dolly-15k & \makecell{Summarization\\Closed QA\\Information Extraction} & Input Context \\
\bottomrule
    \end{tabular}
    \caption{A summary of the RefChecker hallucination detection benchmark. The examples of the benchmark are curated from three different data sources and cover diverse tasks.}
    \label{tab:benchmark_data}
\end{table*}

We assembled a benchmark dataset comprising 300 examples from public datasets, with 100 examples for each of the three settings mentioned in Section~\ref{sec:taxonomy}.  We further collected responses from 7 LLMs on the established benchmark for human evaluation.

\subsection{Curation of Benchmark Data}

These examples are obtained through a process of filtering, sampling and hard case selection. The data sources, tasks and the corresponding references are summarized in Table~\ref{tab:benchmark_data}. We describe them in detail as follows.

\paragraph{Zero Context}

We sample examples from the development set of NaturalQuestions (NQ) \cite{kwiatkowski-etal-2019-natural} for knowledge seeking questions over Wikipedia. During the evaluation, we prompt the question to the models as a closed-book QA task and take the annotated long answer as the reference. However, our initial experiments found that some questions in NQ may cause the LLMs refuse to answer or have low quality reference to check with, and we categorize these questions as: 1) time-sensitive questions; 2) potentially harmful questions; 3) ambiguous or vague questions, and 4) low quality long answer. Thus, we prompted ChatGPT (\texttt{GPT-3.5-Turbo}) to filter out these examples from the development set. The prompts used are described in Appendix~\ref{appendix:data}. 

\paragraph{Noisy Context}
We utilize questions sourced from the validation set of MS MARCO dataset\footnote{We use the 2.1 version of MS MARCO hosted on HuggingFace:  \url{https://huggingface.co/datasets/ms_marco/viewer/v2.1}}\cite{DBLP:conf/nips/NguyenRSGTMD16}. Each question in this dataset is accompanied by a list of documents retrieved from the internet, serving as references. These questions originate from Bing search engine query logs, and the references are found through Bing search, encompassing a broad array of websites. Unlike the factual queries in the NQ dataset, these questions tend to be more open-ended (e.g. "How do I use diatomaceous earth to kill roaches?" or "Why is sodium chlorate useful?"). These questions lack definitive references, making it essential to rely on retrieved external sources when crafting responses. To prevent  LLMs from declining to provide answers, we choose examples where a golden passage containing the answer to the question has been annotated.

\paragraph{Accurate Context}
We employ the databricks-dolly-15k instruction tuning dataset\footnote{databricks-dolly-15k dataset is hosted on HuggingFace: \url{https://huggingface.co/datasets/databricks/databricks-dolly-15k}} which serves the purpose of fine-tuning the Dolly LLMs\cite{DatabricksBlog2023DollyV2}. We take its subset of examples that involve closed QA, summarization, and information extraction from a given document which offers an ideal resource for evaluating the Accurate Context scenario.

During the response collection for benchmarking, we use fixed prompt templates in each task setting for collecting responses from LLMs for fair comparisons. For Zero Context setting, the prompt for response collection is the question itself. For Noisy and Accurate Context settings, we use prompt templates shown in Figure~\ref{fig:response_collection_prompts}.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/response_collection_prompts.pdf}
    \caption{Prompt templates for response collection from LLMs on our benchmark. For Zero Context setting, we just use the question itself as the prompt.}
    \label{fig:response_collection_prompts}
\end{figure}

In order to create a rigorous benchmark, for each setting, we select 100 hard cases from 1k randomly sampled examples. We employ a response-level hallucination checker for this selection. Please refer to Appendix~\ref{appendix:hard_case_selection} for details. 

\subsection{Human Evaluation}

We performed a human evaluation of responses generated by seven LLMs on this benchmark dataset, including GPT-4, GPT-3.5-Turbo, InstructGPT, Claude 2, Llama 2 70B Chat, Falcon 40B Instruct and Alpaca 7B. The process involves three steps: gathering responses, extracting claim-triplets with Claude 2 extractor, and asking human annotators to evaluate these claim-triplets. We totally annotated 11k claim-triplets for the 2.1k responses. 23\% of the claim-triplets were double annotated, with 95.0\% Inter-Annotator Agreement. See Appendix~\ref{appendix:annotation} for the details of the annotation process and Appendix~\ref{appendix:observation_from_human_eval} for the analysis of the human evaluation results.


